The human side of Software Engineering Teams: an investigation of contemporary challenges

There have been recent calls for research on the human side of software engineering and its impact on various factors such as productivity, developer happiness and project success. An analysis of which challenges in software engineering teams are most frequent is still missing. We aim to provide a starting point for a theory about relevant human challenges and their causes in software engineering. We establish a reusable set of challenges and start out by investigating the effect of team virtualization. Virtual teams often use digital communication and consist of members with different nationalities. We designed a survey instrument and asked respondents to assess the frequency and criticality of a set of challenges, separated in context "within teams" as well as "between teams and clients", compiled from previous empiric work, blog posts and pilot survey feedback. For the team challenges, we asked if mitigation measures were already in place. Respondents were also asked to provide information about their team setup. The survey also measured Schwartz human values. Finally, respondents were asked if there were additional challenges at their workplace. We report on the results obtained from 192 respondents. We present a set of challenges that takes the survey feedback into account and introduce two categories of challenges; "interpersonal" and "intrapersonal". We found no evidence for links between human values and challenges. We found some significant links between the number of distinct nationalities in a team and certain challenges, with less frequent and critical challenges occurring if 2-3 different nationalities were present compared to a team having members of just one nationality or more than three. A higher degree of virtualization seems to increase the frequency of some human challenges.

==> Appendices/challenge_changelog.tex <==
\section{Changes made to the initial challenge set} \label{appendix_delta}
This is a list of changes that were made to the initial challenges to create the refined problem set, based on feedback in the survey.

The following challenges were \textbf{removed}:
\begin{itemize}
    \item T3 "Lack of teamwork skills", because it was too vague and subject to interpretation.
    \item T4 "Lack of leadership", because it was too vague and could express itself in many ways. The challenges "Lack of mentors", "Lack of mediation in conflict cases", "Demotivation" etc represent the many effects in a more fine-grained manner.
    \item T12 "Insufficient collaboration", because it was too vague.
    \item T17 "Conflicts of interest at management level" because it is too vague, and depending on the interpretation, too close to "Work is not solution-oriented", "Harassment" or "Destructive competition".
    \item T18 "Missing documentation of the project" - not enough of a human challenge. Underlying causes better described with challenges such as T7, T15, T26.
    \item T19 "Information is not made known to the team" - too vague as the challenge depends on who the actor is. It could be missing documentation, bad team coherence, or bad leadership.
    \item T26 "Conflicting working styles" because it was too vague.
    \item T28 "People crying in discussions" removed because it was not seen as relevant in the survey.
\end{itemize}

The following challenges were grouped into a single challenge as they were \textbf{too close in their meaning}:
\begin{itemize}
    \item T6, T25 and T33 merged with T15 "Work is not solution-oriented"
    \item T9, T10, and T11 were merged into one single challenge: "Reluctance to change working habits"
    \item T16 "Language barriers" merged with T20 "Misunderstandings in communication"
    \item T23 "Missing acceptance of alternative lifestyles" merged with T24 "Harassment"
    \item T27 "People getting angry in discussions" merged with new challenge "Aggressive Discussion Styles"
\end{itemize}

The following challenges were \textbf{refined} in their wording:
\begin{itemize}
    \item "Communication plan is neglected" reworded to "Team is not kept up-to-date", as the "plan" specialization is overly specific and other communication issues are better covered by other challenges (such as "Discussions are not solution-oriented").
    \item "Insufficient analysis at the beginning of the task" reworded to "Tasks insufficiently analyzed", to focus more on the actual challenge and remove the temporal component.
    \item "Subjective interpretation of tasks" reworded to "Task is not well defined or explained".
    \item "Misunderstandings in communication" reworded to "Misunderstandings" as it should also cover documentation and anything conveyed via words.
    \item "Certain people dominating discussions" reworded to "Aggressive Discussion Styles" to cover more general discussion issues caused by forceful or aggressive behaviour.
    \item "Missing respect in the workplace" reworded to "Missing appreciation" to distance it from "Harassment" and cover a new aspect.
    \item T32 "Pressure from client forwarded to SE team" generalised to any kind of "Pressure".
\end{itemize}

The following challenges were \textbf{added based on feedback} from the survey:
\begin{itemize}
    \item Different communication preferences
    \item Destructive Competition
    \item Lack of Empathy
    \item Negativity
    \item Lack of mentors
    \item Lack of mediation in conflicts
    \item Bad Work-Life-Balance
    \item Lack of Confidence
    \item Missing team cohesion
    \item Different needs of staff not respected
\end{itemize}

==> Appendices/challenge_descriptions.tex <==
\section{Challenge Descriptions} \label{appendix_challdesc}
\subsection{Interpersonal Challenges}
1. \textbf{“Not my job”-mentality}\newline
People that refuse to take on or help with tasks that are outside of their role or were not explicitly assigned to them during the planning process. Includes situations in which team members stumble across an issue that was not their responsibility, but they could fix with relative ease, yet they choose not to.

2. \textbf{Different communication preferences}\newline
Clashing preferences of how synchronization should happen (chat, mail, voice calls, video calls, in-person meetings, via documentation/planning tools) leading to people being upset over the chosen mode or planning being delayed or obstructed due to unmotivated participation.

3. \textbf{Destructive Competition}\newline
People that put their own personal gain above the common goal. Prestigious tasks are not assigned to the most competent person but out of political reasons. (Representatives of ) departments refusing to cooperate or even manipulating others to profit personally.

4. \textbf{Under-Estimation of skills}\newline
People that systematically underestimate their potential, thus avoiding challenging tasks and potentially limiting their own growth.

5. \textbf{Over-Estimation of skills}\newline
People that systematically overestimate their current skill and knowledge, leading to incorrect time or budget estimates.

6. \textbf{Lack of Empathy}\newline
People without a sense of how those around them feel or without a will to adapt to the emotional state of colleagues. Example: Anxious colleague is yelled at for not being able to complete a task instead of supported. Emotional unrest is not recognized and no support offered by superiors or colleagues.

7. \textbf{Pressure}\newline
People being pressured to be more productive using forceful communication  (yelling, belittling, needlessly pointing out deadlines) instead of jointly looking for ways or getting additional resources to improve the situation.

8. \textbf{People not reporting problems in time}\newline
People not requesting assistance or not reporting a blocking problem immediately, potentially pretending there is no problem as to not lose face, potentially endangering financial or time constraints.

9. \textbf{Frequently changing team members}\newline
The teams are often recomposed and workers have to work with and adapt to new team members.

10. \textbf{Aggressive Discussion Styles}\newline
People that use shouting, yelling and general aggressive verbal modes, or try to allocate a lot of speaking time for themselves, while not giving room to speak for less dominant colleagues.

11. \textbf{Misunderstandings}\newline
The intended meaning is not transferred accurately over the selected communication channel. This could be due to bad pronunciation, language barriers, technical issues, use of sarcasm/irony, leaving out details because it is assumed it is already known etc.

12. \textbf{Discussions are not solution-oriented}\newline
Discussions or meeting often either become off-topic or are not aimed towards finding an actual solution, but rather used as a vent to complain about circumstances.

13. \textbf{Reluctance to change working habits}\newline
Staff are reluctant to try out new infrastructure, processes or tools and would rather stick to the established, even if it is known to perform worse.

14. \textbf{Team is not kept up-to-date}\newline
Updates regarding the project, the team’s or company’s vision, problems and goals or staff changes are not communicated clearly and in time. 

15. \textbf{Lack of mentors}\newline
Delays occur as there is no designated person to contact in case of technical issues or lack of knowledge about company procedures.

16. \textbf{Missing team cohesion}\newline
There is no feeling of being a “closely knit” team, with its members supporting each other technically and emotionally and being interested in each other’s tasks.

17. \textbf{Different needs of staff not respected}\newline
The working environment does not cater to individual needs and requests for individual changes are not respected by the management, leading to colleagues feeling unhappy about the place they work in. Examples: Standing desks are denied. People are forced to work in open space offices.

18. \textbf{Negativity}\newline
A general sense of negativity lingers, causing demotivation and rants rather than a productive spirit of problem solving.

19. \textbf{Harassment}\newline
People harassing colleagues, including insults, threats, belittling, lack of respect, racism and sexism. 

20. \textbf{Missing appreciation}\newline
Superiors or colleagues rarely acknowledge the work behind a successful task, or the sacrifices individual staff made to make something possible.

21. \textbf{Lack of mediation in conflicts}\newline
Personal disputes linger on for a long time, potentially disrupting productivity, as there is no procedure or responsible person to mediate the two opposing parties. 
\subsection{Intrapersonal Challenges}
1. \textbf{Bad Work-Life-Balance}\newline
Unmitigated fatigue leading to less productivity during work hours.

2. \textbf{Work is not solution-oriented}\newline
A lot of time is spent on work that does not add to the solution, but is necessary to meet a certain (potentially emotional) expectation. Example: A certain style of code is required even though the delivered code meets quality and maintainability standards. An unsuitable framework is used because a team lead prefers it.

3. \textbf{Tasks insufficiently analyzed}\newline
The complexity and requirements of a task were not explored well enough, thus leading to an incorrect time assessment or lack of required knowledge to solve it well and in time.

4. \textbf{Task is not well defined or explained}\newline
Tasks are often not explained sufficiently, leave too much room for interpretation, possibly leading to unnecessary or wrong implementations that need to be revised later on.

5. \textbf{Lack of knowledge}\newline
The assigned tasks require far more expertise than the assignee has. While a challenging task can lead to growth, a task that is by far too difficult can hinder learning (Zone of proximal development).

6. \textbf{Gold Plating}\newline
Tasks are “overdone” and more functionality than required by the task or client is added.

7. \textbf{Demotivation}\newline
Time is wasted and procrastination occurs as there is a feeling of not wanting to work on specific tasks.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************

